Finite free convolutions of polynomials

We study three convolutions of polynomials in the context of free probability theory. We prove that these convolutions can be written as the expected characteristic polynomials of sums and products of unitarily invariant random matrices. The symmetric additive and multiplicative convolutions were introduced by Walsh and Szeg\"o in different contexts, and have been studied for a century. The asymmetric additive convolution, and the connection of all of them with random matrices, is new. By developing the analogy with free probability, we prove that these convolutions produce real rooted polynomials and provide strong bounds on the locations of the roots of these polynomials.

==> notation.tex <==

\begin{tabular}{l | l | l}
Notation & Latex & Meaning\\
\hline
$\sqsum $ & \texttt{\textbackslash sqsum}  & additive symmetric (square) convolution
\\
$\recsum $ & \texttt{\textbackslash recsum}  & additive asymmetric  (rectangular) convolution
\\
$\sqmult$ &  \texttt{\textbackslash sqmult}  & multiplicative convolution
\\
$\charp{x}{M}$ & \texttt{\textbackslash charp\{x\}\{M\}}
& characteristic poly of $M$ in $x$ \\
$\cauchy{p}{x}$ & \texttt{\textbackslash cauchy\{p\}\{x\}} & the Cauchy/Stieltjes transform\\
$\invcauchy{p}{x}$ & \texttt{\textbackslash invcauchy\{p\}\{x\}} & the inverse Cauchy/Stieltjes transform (not sure I like $\mathcal{G}$)\\
$\rtrans{p}{x}$  & \texttt{\textbackslash rtrans\{p\}\{x\}} & the Voiculescu R-transform\\
$\reccauchy{p}{x}$ & \texttt{\textbackslash reccauchy\{p\}\{x\}} & analog of Cauchy for rectangular (nonstandard)\\
$\invreccauchy{p}{x}$ & \texttt{\textbackslash invreccauchy\{p\}\{x\}} & analog of inverse Cauchy for asymmetric (nonstandard)\\
$\rectrans{p}{x}$  & \texttt{\textbackslash rectrans\{p\}\{x\}} & analog of  R-transform for rectangular (nonstandard)\\
$\subsquare$ & \texttt{\textbackslash subsquare} & $\subsquare p (x) = p (x^{2})$\\
$\deriv$ & \texttt{\textbackslash deriv} & the derivative\\
$\shiftoper{t}$ & \texttt{\textbackslash shiftoper\{t\}} & the operator $I - t D$\\
$\maxroot{p}$ & \texttt{\textbackslash maxroot\{p\}} & the largest root of the polynomial\\
$\rrpoly{d}$ & \texttt{\textbackslash rrpoly\{d\}} & real rooted polynomials of degree $d$, positive leading coefficient\\
$\rrpos{d}$ & \texttt{\textbackslash rrpos\{d\}} & nonnegative rooted polynomials of degree $d$, positive leading coefficient\\
\end{tabular}


